Decentralized optimization with affine constraints over time-varying networks

The decentralized optimization paradigm assumes that each term of a finite-sum objective is privately stored by the corresponding agent. Agents are only allowed to communicate with their neighbors in the communication graph. We consider the case when the agents additionally have local affine constraints and the communication graph can change over time. We provide the first linearly convergent decentralized algorithm for time-varying networks by generalizing the optimal decentralized algorithm ADOM to the case of affine constraints. We show that its rate of convergence is optimal for first-order methods by providing the lower bounds for the number of communications and oracle calls.

==> adomplus_draft.tex <==
\subsection{Application of ADOM+}
Initial ADOM+ reformulation is $(\cA+\cB) (x, y, z) = 0$, where
\begin{equation}
\cA(x, y, z)= \begin{bmatrix}
\nabla F(x)-\nu x \\
\nu^{-1}(y+z) \\
\mathbf{P} \nu^{-1}(y+z) \end{bmatrix}, 
\quad 
\cB(x, y, z)=\begin{bmatrix}
-y \\
x \\
0 \end{bmatrix}.
\end{equation}

In case of common constraints, it could be extended to
\begin{equation}
\cA(x, y, z, u)= \begin{bmatrix}
\nabla F(x)-\nu x \\
\nu^{-1}(y+z+\bA^\top u) \\
\mathbf{P} \nu^{-1}(y+z+\bA^\top u) \\
\bA \nu^{-1} (y+z+\bA^\top u)  
\end{bmatrix}, 
\quad 
\cB(x, y, z, u)=\begin{bmatrix}
-y \\ x \\ 0 \\ \bb \\ 
\end{bmatrix}.
\end{equation}

For convenience we define $v = v(y,z,u) = y + z+ \mAT u$ and $v^* = v(y^*, z^*, u^*)$. 
Then $(\cA+\cB) (x^*, y^*, z^*, u^*) = 0$ corresponds to four optimality conditions: 
\begin{align}
0&= \g F(x^*)  - \nu x^* - y^*,\label{opt:x}\\
0&= \nu^{-1}v^*  + x^*,\label{opt:y}\\
\cL &\ni v^*,\label{opt:z}\\
0&= \nu^{-1}\mA v^* + \bb.\label{opt:u}
\end{align}

After replacing $\bP$ with its inexact analog $\bW$, ADOM+ algorithm is composed by combining Forward-Backward (FB) algorithm + Error-Feedback (EF) on $z$ + Nesterov's acceleration (не очевидно, как именно вставляется).  
\begin{algorithm}[H]
	% \caption{\algname{ADOM+}}
	\caption{ADOM+ with common affine constraints}
	\label{scary:alg}
	\begin{algorithmic}[1]
		\STATE {\bf input:} $x^0, y^0,m^0 \in (\R^d)^\cV$, $z^0 \in \cL^\perp$
		\STATE $x_f^0 = x^0$, $y_f^0 = y^0$, $z_f^0 = z^0$
		\FOR{$k = 0,1,2,\ldots$}
		% \STATE $v^k_g = y_g^k + z_g^k + \mAT u_g^k$ \label{scary:line:v}  % ro in ipynb
		\STATE $v^k_g = y_g^k + z_g^k$ \label{scary:line:v}  % ro in ipynb
		\STATE $x_g^k = \tau_1x^k + (1-\tau_1) x_f^k$\label{scary:line:x:1}
		\STATE $x^{k+1} = x^k + \eta\alpha(x_g^k - x^{k+1}) - \eta\left[\g F(x_g^k) - \nu x_g^k - y^{k+1}\right] $\label{scary:line:x:2}
		\STATE $x_f^{k+1} = x_g^k + \tau_2 (x^{k+1} - x^k)$\label{scary:line:x:3}
		
		\STATE $y_g^k = \sigma_1 y^k + (1-\sigma_1)y_f^k$\label{scary:line:y:1}
		\STATE $y^{k+1} = y^k + \theta\beta (\g F(x_g^k   ) - \nu x_g^k - y^{k+1}) -\theta\left[\nu^{-1}v^k_g + x^{k+1}\right]$\label{scary:line:y:2}
		\STATE $y_f^{k+1} = y_g^k + \sigma_2 (y^{k+1} - y^k)$\label{scary:line:y:3}
		
		\STATE $z_g^k = \sigma_1 z^k + (1-\sigma_1)z_f^k$\label{scary:line:z:1}
        \STATE $s^k = \left(\nu^{-1}\mBT\mB v^k_g + \mBT \bb \right)$
		\STATE $z^{k+1} = z^k + \gamma \delta(z_g^k - z^k) - \mW(k)\left[\gamma s^k + m^k\right]$\label{scary:line:z:2}
		\STATE $m^{k+1} = \gamma s^k + m^k - \mW(k)\left[\gamma s^k + m^k\right]$\label{scary:line:m}
		\STATE $z_f^{k+1} = z_g^k - \zeta \left( \mW(k) \mBT \mB v_g^k + \nu \mBT \bb \right)$ \label{scary:line:z:3}
  
        % \STATE $u^k_g = \sigma_1 u^k + (1 - \sigma_1) u^k_f$ \label{scary:line:u_g}
        % \STATE $u^{k+1} = u^k + \gamma_u \delta_u (u^k_g - u^k) - \gamma_u(\nu^{-1}\mA v^k_g  + \bb)$\label{scary:line:u}
        % \STATE $u^{k+1}_f = u^k_g - \zeta_u (\nu^{-1}\mA v^k_g + \bb)$\label{scary:line:u_f}
		\ENDFOR
	\end{algorithmic}
\end{algorithm}

\begin{enumerate}
	\item $\mW(q)_{i,j} \neq 0$  if and only if $(i,j) \in \cE^q$ or $i=j$,
	%\item $\mW(q)  \ones_n= \zeros_n$, $\ones_n^\top \mW(q) = \zeros_n^\top$, where $\ones_n = (1,\ldots,1) \in \R^n$, $\zeros_n = (0,\ldots,0) \in \R^n$,
	\item $\ker \mW(q) \supset  \left\{ (x_1,\ldots,x_n) \in \R^n : x_1 = \ldots = x_n \right\}$,
	\item $\range \mW(q) \subset \left\{(x_1,\ldots,x_n) \in\R^n : \sum_{i=1}^n x_i = 0\right\}$,
	\item There exists $\chi \geq 1$, such that 
	\begin{equation}\label{eq:chi}
		\sqn{\mW x - x} \leq (1-\chi^{-1})\sqn{x} \text{ for all } x  \in \left\{ (x_1,\ldots,x_n) \in \R^n :\sum_{i =1}^n x_i = 0\right\}.
	\end{equation}	
\end{enumerate}


Let us define $v^k, v_f^k, v_g^k$ = ...

\begin{lemma}
    (Lemma 5)
	Let $\beta$ be defined as follows:
	\begin{equation}\label{scary:beta}
	\beta = 1/(2L).
	\end{equation}
	Let $\sigma_1$ be defined as follows:
	\begin{equation}\label{scary:sigma1}
	\sigma_1 = (1/\sigma_2 + 1/2)^{-1}.
	\end{equation}
	Then the following inequality holds:
	\begin{equation}
	\begin{split}\label{scary:eq:y}
	\MoveEqLeft[4]
	\left(\frac{1}{\theta} + \frac{\beta}{2}\right)\sqn{y^{k+1} - y^*}
	+
	\frac{\beta}{2\sigma_2}\sqn{y_f^{k+1} - y^*}\\
	&\leq
	\frac{1}{\theta}\sqn{y^k - y^*}
	+
	\frac{\beta(1-\sigma_2/2)}{2\sigma_2}\sqn{y_f^k - y^*}
	+
	\bg_F(x_g^k, x^*) - \frac{\nu}{2}\sqn{x_g^k - x^*}
	-
	2\<x^{k+1} - x^*, y^{k+1} - y^*>
	\\&-
	2\nu^{-1}\<v_g^k -  v^*, y^{k+1} - y^*>
	-
	\frac{\beta}{4}\sqn{y_g^k - y^*}
	+
	\left(\frac{\beta\sigma_2^2}{4} - \frac{1}{\theta}\right)\sqn{y^{k+1} - y^k}.
	\end{split}
	\end{equation}
\end{lemma}
\begin{proof}
    The proof is the same as of the original Lemma, one just need to replace $y_g^k + z_g^k$ with $v_g^k$ and $y^* + z^*$ with $v^*$ everywhere in the original proof. 
\end{proof}

\begin{lemma}
    (Lemma 6)
	The following inequality holds:
	\begin{equation}\label{scary:eq:2}
	\sqn{m^k}_\mP
	\leq
	8\chi^2\gamma^2\nu^{-2}\sqn{v^k_g}_\mP + 4\chi(1 - (4\chi)^{-1})\sqn{m^k}_\mP - 4\chi\sqn{m^{k+1}}_\mP.
	\end{equation}
\end{lemma}
\begin{proof}
	Using Line~\ref{scary:line:m} of Algorithm~\ref{scary:alg} we get
	\begin{align*}
	\sqn{m^{k+1}}_\mP
	&=
	\sqn{\gamma\nu^{-1}v^k_g + m^k - (\mW(k)\otimes \mI_d)\left[\gamma\nu^{-1}v^k_g + m^k\right]}_{\mP}\\
	&=
	\sqn{\mP\left[\gamma\nu^{-1}v^k_g + m^k\right]- (\mW(k)\otimes \mI_d)\mP\left[\gamma\nu^{-1}v^k_g + m^k\right]}.
	\end{align*}
	Using  property \eqref{eq:chi} we obtain
	\begin{align*}
	\sqn{m^{k+1}}_\mP
	&\leq (1 - \chi^{-1})
	\sqn{m^k + \gamma\nu^{-1}v^k_g}_\mP.
	\end{align*}
	Using inequality $\sqn{a+b} \leq (1+c)\sqn{a} + (1+c^{-1})\sqn{b}$ with $c = \frac{1}{2(\chi - 1)}$ we get
	\begin{align*}
	\sqn{m^{k+1}}_\mP
	&\leq (1 - \chi^{-1})
	\left[
	\left(1 + \frac{1}{2(\chi - 1)}\right)\sqn{m^k}_\mP
	+ 
	\left(1 +  2(\chi - 1)\right)\gamma^2\nu^{-2}\sqn{v^k_g}_\mP
	\right]
	\\&\leq
	(1 - (2\chi)^{-1})\sqn{m^k}_\mP
	+
	2\chi\gamma^2\nu^{-2}\sqn{v^k_g}_\mP.
	\end{align*}
	Rearranging gives
	\begin{align*}
	\sqn{m^k}_\mP
	&\leq
	8\chi^2\gamma^2\nu^{-2}\sqn{v^k_g}_\mP + 4\chi(1 - (4\chi)^{-1})\sqn{m^k}_\mP - 4\chi\sqn{m^{k+1}}_\mP.
	\end{align*}
\end{proof}

\begin{lemma} (Lemma 7)
	Let $\z^k$ be defined as follows:
	\begin{equation}\label{scary:zhat}
	\z^k = z^k - \mP m^k.
	\end{equation}
	Then the following inequality holds:
	\begin{equation}
	\begin{split}\label{scary:eq:z}
	\MoveEqLeft[4]\frac{1}{\gamma}\sqn{\z^{k+1} - z^*}
	+
	\frac{4}{3\gamma}\sqn{m^{k+1}}_\mP
	\leq
	\left(\frac{1}{\gamma} - \delta\right)\sqn{\z^k - z^*}
	+
	\left(1-(4\chi)^{-1} +\frac{3\gamma\delta}{2}\right)\frac{4}{3\gamma}\sqn{m^k}_\mP
	\\&-
	2\nu^{-1}\<v^k_g - v^*,z^k - z^*>
	+
	\gamma\nu^{-2}\left(1 + 6\chi\right)\sqn{v^k_g}_\mP
	\\&+
	2\delta\sqn{z_g^k  - z^*}
	+
	\left(2\gamma\delta^2-\delta\right)\sqn{z_g^k - z^k}.
	\end{split}
	\end{equation}
\end{lemma}
\begin{proof}
	\begin{align*}
	\frac{1}{\gamma}\sqn{\z^{k+1} - z^*}
	&=
	\frac{1}{\gamma}\sqn{\z^k - z^*}
	+
	\frac{2}{\gamma}\<\z^{k+1} - \z^k,\z^k - z^*>
	+
	\frac{1}{\gamma}\sqn{\z^{k+1} - \z^k}.
	\end{align*}
	Lines~\ref{scary:line:z:2} and~\ref{scary:line:m} of Algorithm~\ref{scary:alg} together with $\z^k$ definition \eqref{scary:zhat} imply
	\begin{equation*}
	\z^{k+1} - \z^k = \gamma\delta(z_g^k - z^k) - \gamma\nu^{-1}\mP v^k_g.
	\end{equation*}
	Hence,
	\begin{align*}
	\frac{1}{\gamma}\sqn{\z^{k+1} - z^*}
	&=
	\frac{1}{\gamma}\sqn{\z^k - z^*}
	+
	2\delta\<z_g^k - z^k,\z^k - z^*>
	-
	2\nu^{-1}\<\mP v^k_g,\z^k - z^*>
	+
	\frac{1}{\gamma}\sqn{\z^{k+1} - \z^k}
	\\&=
	\frac{1}{\gamma}\sqn{\z^k - z^*}
	+
	\delta\sqn{z_g^k - \mP m^k - z^*} - \delta\sqn{\z^k - z^*} - \delta\sqn{z_g^k - z^k}
	\\&-
	2\nu^{-1}\<\mP v^k_g,\z^k - z^*>
	+
	\gamma\sqn{\delta(z_g^k - z^k) - \nu^{-1}\mP v^k_g}
	\\&\leq
	\left(\frac{1}{\gamma} - \delta\right)\sqn{\z^k - z^*}
	+
	2\delta\sqn{z_g^k  - z^*}
	+
	2\delta\sqn{m^k}_\mP
	-
	\delta\sqn{z_g^k - z^k}
	\\&-
	2\nu^{-1}\<\mP v^k_g,\z^k - z^*>
	+
	2\gamma\delta^2\sqn{z_g^k - z^k}
	+
	\gamma\sqn{\nu^{-1}\mP v^k_g}
	\\&\leq
	\left(\frac{1}{\gamma} - \delta\right)\sqn{\z^k - z^*}
	+
	2\delta\sqn{z_g^k  - z^*}
	+
	\left(2\gamma\delta^2-\delta\right)\sqn{z_g^k - z^k}
	\\&-
	2\nu^{-1}\<\mP v^k_g,z^k - z^*>
	+
	\gamma\sqn{\nu^{-1}\mP v^k_g}
	+
	2\delta\sqn{m^k}_\mP
	+
	2\nu^{-1}\<\mP v^k_g,m^k>.
	\end{align*}
	Using the fact that $z^k \in \cL^\perp$ for all $k=0,1,2\ldots$ and optimality condition \eqref{opt:z} we get
	\begin{align*}
	\frac{1}{\gamma}\sqn{\z^{k+1} - z^*}
	&\leq
	\left(\frac{1}{\gamma} - \delta\right)\sqn{\z^k - z^*}
	+
	2\delta\sqn{z_g^k  - z^*}
	+
	\left(2\gamma\delta^2-\delta\right)\sqn{z_g^k - z^k}
	\\&-
	2\nu^{-1}\<v^k_g - (y^*+z^*),z^k - z^*>
	+
	\gamma\nu^{-2}\sqn{v^k_g}_\mP
	\\&+
	2\delta\sqn{m^k}_\mP
	+
	2\nu^{-1}\<\mP v^k_g,m^k>.
	\end{align*}
	Using Young's inequality we get
	\begin{align*}
	\frac{1}{\gamma}\sqn{\z^{k+1} - z^*}
	&\leq
	\left(\frac{1}{\gamma} - \delta\right)\sqn{\z^k - z^*}
	+
	2\delta\sqn{z_g^k  - z^*}
	+
	\left(2\gamma\delta^2-\delta\right)\sqn{z_g^k - z^k}
	\\&-
	2\nu^{-1}\<v^k_g - v^*,z^k - z^*>
	+
	\gamma\nu^{-2}\sqn{v^k_g}_\mP
	\\&+
	2\delta\sqn{m^k}_\mP
	+
	3\gamma\chi\nu^{-2}\sqn{v^k_g}_\mP + \frac{1}{3\gamma\chi}\sqn{m^k}_\mP.
	\end{align*}
	Using \eqref{scary:eq:2} we get
	\begin{align*}
	\frac{1}{\gamma}\sqn{\z^{k+1} - z^*}
	&\leq
	\left(\frac{1}{\gamma} - \delta\right)\sqn{\z^k - z^*}
	+
	2\delta\sqn{z_g^k  - z^*}
	+
	\left(2\gamma\delta^2-\delta\right)\sqn{z_g^k - z^k}
	\\&-
	2\nu^{-1}\<v^k_g - v^*,z^k - z^*>
	+
	\gamma\nu^{-2}\sqn{v^k_g}_\mP
	\\&+
	2\delta\sqn{m^k}_\mP
	+
	6\gamma\nu^{-2}\chi\sqn{v^k_g}_\mP + \frac{4(1 - (4\chi)^{-1})}{3\gamma}\sqn{m^k}_\mP - \frac{4}{3\gamma}\sqn{m^{k+1}}_\mP
	\\&=
	\left(\frac{1}{\gamma} - \delta\right)\sqn{\z^k - z^*}
	+
	2\delta\sqn{z_g^k  - z^*}
	+
	\left(2\gamma\delta^2-\delta\right)\sqn{z_g^k - z^k}
	\\&-
	2\nu^{-1}\<v^k_g - v^*,z^k - z^*>
	+
	\gamma\nu^{-2}\left(1 + 6\chi\right)\sqn{v^k_g}_\mP
	\\&+
	\left(1-(4\chi)^{-1}+\frac{3\gamma\delta}{2}\right)\frac{4}{3\gamma}\sqn{m^k}_\mP - \frac{4}{3\gamma}\sqn{m^{k+1}}_\mP.
	\end{align*}
\end{proof}

\begin{lemma} (Lemma 7 + NEW LEMMA DRAFTTT)
	Let $\z^k$ be defined as follows:
	\begin{equation}\label{scary:zhat}
	\z^k = z^k - \mP m^k.
	\end{equation}
    Assume $\delta_u = \delta,~ \gamma_u = \gamma$.
	Then the following inequality holds:
	\begin{equation}
 ?????
	\begin{split}\label{scary:eq:zu}
	\MoveEqLeft[8] \frac{1}{\gamma}\sqn{(\z^{k+1} - z^*) + \mAT(u^{k+1} - u^*)}
	+
	\frac{4}{3\gamma}\sqn{m^{k+1}}_\mP
	\\&\leq
	\left(\frac{1}{\gamma} - \delta\right)\sqn{(\z^{k} - z^*) + (u^{k} - u^*)}
	+
	2\delta\sqn{(z_g^{k} - z^*) + (u_g^{k} - u^*)}
    \\&+
	\left(2\gamma\delta^2 - \delta\right)\sqn{(\z_g^{k} - z^k) + (u_g^{k} - u^k)}
    +
	\left(1-(4\chi)^{-1} +\frac{3\gamma\delta}{2}\right)\frac{4}{3\gamma}\sqn{m^k}_\mP
	\\&-
	2\nu^{-1}\<v^k_g - v^*,z^k - z^* + \mAT (u^k - u^*)>
	+
	\gamma\nu^{-2}\left(6\chi + 4 + \frac\nu\gamma \right)\sqn{v^k_g}_\mP
	\\&+
    \nu^{-1} \sqn{u^k - u^*}
    +
    \nu^{-1} \sqn{\z^k - z^*}
    + \left(4 \gamma + \nu \right) \sqn{\nu^{-1}\mA v_g^k + \bb}
	\end{split}
	\end{equation}
\end{lemma}
\begin{proof}
	\begin{align*}
	\frac{1}{\gamma}\sqn{(\z^{k+1} - z^*) + (u^{k+1} - u^*)}
	&=
	\frac{1}{\gamma}\sqn{(\z^k - z^*) + (u^k - u^*)}
	+
	\frac{1}{\gamma}\sqn{(\z^{k+1} - \z^k) + (u^{k+1} - u^k)}
	\\&+
	\frac{2}{\gamma}\<(\z^{k+1} - \z^k) + (u^{k+1} - u^k),(\z^k - z^*) + (u^k - u^*)>
    .
	\end{align*}
	Lines~\ref{scary:line:z:2} and~\ref{scary:line:m} of Algorithm~\ref{scary:alg} together with $\z^k$ definition \eqref{scary:zhat} imply
	\begin{equation*}
	\z^{k+1} - \z^k = \gamma\delta(z_g^k - z^k) - \gamma\nu^{-1}\mP v^k_g.
	\end{equation*}
	Hence,
	% \begin{align*}
	% &\frac{1}{\gamma}\sqn{(\z^{k+1} - z^*) + (u^{k+1} - u^*)}
	% \\&=
	% \frac{1}{\gamma}\sqn{\z^k - z^*}
	% +
	% 2\delta\<z_g^k - z^k,\z^k - z^*>
	% -
	% 2\nu^{-1}\<\mP v^k_g,\z^k - z^*>
	% +
	% \frac{1}{\gamma}\sqn{\z^{k+1} - \z^k}
	% \\&=
	% \frac{1}{\gamma}\sqn{\z^k - z^*}
	% +
	% \delta\sqn{z_g^k - \mP m^k - z^*} - \delta\sqn{\z^k - z^*} - \delta\sqn{z_g^k - z^k}
	% \\&-
	% 2\nu^{-1}\<\mP v^k_g,\z^k - z^*>
	% +
	% \gamma\sqn{\delta(z_g^k - z^k) - \nu^{-1}\mP v^k_g}
	% \\&\leq
	% \left(\frac{1}{\gamma} - \delta\right)\sqn{\z^k - z^*}
	% +
	% 2\delta\sqn{z_g^k  - z^*}
	% +
	% 2\delta\sqn{m^k}_\mP
	% -
	% \delta\sqn{z_g^k - z^k}
	% \\&-
	% 2\nu^{-1}\<\mP v^k_g,\z^k - z^*>
	% +
	% 2\gamma\delta^2\sqn{z_g^k - z^k}
	% +
	% \gamma\sqn{\nu^{-1}\mP v^k_g}
	% \\&\leq
	% \left(\frac{1}{\gamma} - \delta\right)\sqn{\z^k - z^*}
	% +
	% 2\delta\sqn{z_g^k  - z^*}
	% +
	% \left(2\gamma\delta^2-\delta\right)\sqn{z_g^k - z^k}
	% \\&-
	% 2\nu^{-1}\<\mP v^k_g,z^k - z^*>
	% +
	% \gamma\sqn{\nu^{-1}\mP v^k_g}
	% +
	% 2\delta\sqn{m^k}_\mP
	% +
	% 2\nu^{-1}\<\mP v^k_g,m^k>.
	% \end{align*}
	% Using the fact that $z^k \in \cL^\perp$ for all $k=0,1,2\ldots$ and optimality condition \eqref{opt:z} we get
	% \begin{align*}
	% \frac{1}{\gamma}\sqn{\z^{k+1} - z^*}
	% &\leq
	% \left(\frac{1}{\gamma} - \delta\right)\sqn{\z^k - z^*}
	% +
	% 2\delta\sqn{z_g^k  - z^*}
	% +
	% \left(2\gamma\delta^2-\delta\right)\sqn{z_g^k - z^k}
	% \\&-
	% 2\nu^{-1}\<v^k_g - (y^*+z^*),z^k - z^*>
	% +
	% \gamma\nu^{-2}\sqn{v^k_g}_\mP
	% \\&+
	% 2\delta\sqn{m^k}_\mP
	% +
	% 2\nu^{-1}\<\mP v^k_g,m^k>.
	% \end{align*}
	% Using Young's inequality we get
	% \begin{align*}
	% \frac{1}{\gamma}\sqn{\z^{k+1} - z^*}
	% &\leq
	% \left(\frac{1}{\gamma} - \delta\right)\sqn{\z^k - z^*}
	% +
	% 2\delta\sqn{z_g^k  - z^*}
	% +
	% \left(2\gamma\delta^2-\delta\right)\sqn{z_g^k - z^k}
	% \\&-
	% 2\nu^{-1}\<v^k_g - v^*,z^k - z^*>
	% +
	% \gamma\nu^{-2}\sqn{v^k_g}_\mP
	% \\&+
	% 2\delta\sqn{m^k}_\mP
	% +
	% 3\gamma\chi\nu^{-2}\sqn{v^k_g}_\mP + \frac{1}{3\gamma\chi}\sqn{m^k}_\mP.
	% \end{align*}
	% Using \eqref{scary:eq:2} we get
	% \begin{align*}
	% \frac{1}{\gamma}\sqn{\z^{k+1} - z^*}
	% &\leq
	% \left(\frac{1}{\gamma} - \delta\right)\sqn{\z^k - z^*}
	% +
	% 2\delta\sqn{z_g^k  - z^*}
	% +
	% \left(2\gamma\delta^2-\delta\right)\sqn{z_g^k - z^k}
	% \\&-
	% 2\nu^{-1}\<v^k_g - v^*,z^k - z^*>
	% +
	% \gamma\nu^{-2}\sqn{v^k_g}_\mP
	% \\&+
	% 2\delta\sqn{m^k}_\mP
	% +
	% 6\gamma\nu^{-2}\chi\sqn{v^k_g}_\mP + \frac{4(1 - (4\chi)^{-1})}{3\gamma}\sqn{m^k}_\mP - \frac{4}{3\gamma}\sqn{m^{k+1}}_\mP
	% \\&=
	% \left(\frac{1}{\gamma} - \delta\right)\sqn{\z^k - z^*}
	% +
	% 2\delta\sqn{z_g^k  - z^*}
	% +
	% \left(2\gamma\delta^2-\delta\right)\sqn{z_g^k - z^k}
	% \\&-
	% 2\nu^{-1}\<v^k_g - v^*,z^k - z^*>
	% +
	% \gamma\nu^{-2}\left(1 + 6\chi\right)\sqn{v^k_g}_\mP
	% \\&+
	% \left(1-(4\chi)^{-1}+\frac{3\gamma\delta}{2}\right)\frac{4}{3\gamma}\sqn{m^k}_\mP - \frac{4}{3\gamma}\sqn{m^{k+1}}_\mP.
	% \end{align*}
\end{proof}


\begin{lemma}
    (Lemma 8)
	The following inequality holds:
	\begin{equation}
	\begin{split}\label{scary:eq:3}
	2\<v_g^k - v^*, v^k - v^*>
	\\&\geq
	2\sqn{v_g^k - v^*}
	+
	\frac{(1-\sigma_2/2)}{\sigma_2}\left(\sqn{v_g^k - v^*}  - \sqn{v_f^k - v^*}\right).
	\end{split}
	\end{equation}
\end{lemma}
\begin{proof}
	\begin{align*}
	\MoveEqLeft[4]2\<v_g^k - (v^*), v^k - v^*>
	\\&=
	2\sqn{v_g^k - v^*}
	+
	2\<v_g^k - v^*, v^k - v_g^k>.
	\end{align*}
	Using Lines~\ref{scary:line:y:1}, \ref{scary:line:z:1} and~\ref{scary:line:u_g} of Algorithm~\ref{scary:alg} we get
	\begin{align*}
	\MoveEqLeft[4]2\<v_g^k - v^*,v^k - v^*>
	\\&=
	2\sqn{v_g^k - v^*}
	+
	\frac{2(1-\sigma_1)}{\sigma_1}\<v_g^k - v^*, v_g^k - v_f^k>
	\\&=
	2\sqn{v_g^k - v^*}
	\\&+
	\frac{(1-\sigma_1)}{\sigma_1}\left(\sqn{v_g^k - v^*} + \sqn{v_g^k - v_f^k} - \sqn{v_f^k - v^*}\right)
	\\&\geq
	2\sqn{v_g^k - v^*}
	+
	\frac{(1-\sigma_1)}{\sigma_1}\left(\sqn{v^k - v^*}  - \sqn{v_f^k - v^*}\right).
	\end{align*}
	Using $\sigma_1$ definition $\sigma_1 = (1/\sigma_2 + 1/2)^{-1}$ we get
	\begin{align*}
	\MoveEqLeft[4]2\<v_g^k - v^* ,v^k - v^*>
	\\&\geq
	2\sqn{v_g^k - v^*}
	+
	\frac{(1-\sigma_2/2)}{\sigma_2}\left(\sqn{v_g^k - v^*}  - \sqn{v_f^k - v^*}\right).
	\end{align*}
\end{proof}



\begin{lemma}
    (Lemma 9)
	Let $\zeta$ be defined by
	\begin{equation}\label{scary:zeta}
	\zeta = 1/3,
	\end{equation}
    and let $\mP_A$ be the projector on $\image \mA$.
	Then the following inequality holds:
	\begin{equation}
	\begin{split}\label{scary:eq:4}
	\MoveEqLeft[6]-
	2\<y^{k+1} - y^k,v_g^k - v^*>
	\\&\leq
	\frac1{\sigma_2}\sqn{v_g^k - v^*}
    -
    \newu{\frac1{3\sigma_2\chitA} \sqn{(v_g^k - v^*)}_{\mP_A} }
    - 
	\frac1{\sigma_2}\sqn{v_f^{k+1} - v^*}
	\\&+
	3\sigma_2\sqn{y^{k+1} - y^k}
	-
    \frac1{3\sigma_2\chi} \sqn{v_g^k}_\mP
	\end{split}
	\end{equation}
\end{lemma}
\begin{proof}
	\begin{align*}
	\sqn{v_f^{k+1} - v^*}
	&=
	\sqn{v_g^k - v^*} + 2\<v_f^{k+1} - v_g^k, v_g^k - v^*>
	+
	\sqn{v_f^{k+1} - v_g^k}
	\\&\leq
	\sqn{v_g^k - v^*} + 2\<v_f^{k+1} - v_g^k,v_g^k - v^*>
	\\&+
	\newu3\sqn{y_f^{k+1} - y_g^k}
	+
	\newu3\sqn{z_f^{k+1} - z_g^k}
    +  
    \newu{3\sqn{\mAT (u_f^{k+1} - u_g^k)}}.
	\end{align*}
	Using Line~\ref{scary:line:y:3} of Algorithm~\ref{scary:alg} we get
	\begin{align*}
	\sqn{v_f^{k+1} - v^*}
	&\leq
	\sqn{v_g^k - v^*}
	+
	2\sigma_2\<y^{k+1} - y^k,v_g^k - v^*>
	+
	3\sigma_2^2\sqn{y^{k+1} - y^k}
	\\&+
	2\<z_f^{k+1} - z_g^k,v_g^k - v^*>
	+
    \newu{2\<\mAT (u_f^{k+1} - u_g^k),v_g^k - v^*>}
    \\&+
	3\sqn{z_f^{k+1} - z_g^k}
    + 
    \newu{3\sqn{\mAT (u_f^{k+1} - u_g^k)}}.
	\end{align*}
	Using Lines~\ref{scary:line:z:3} and~\ref{scary:line:u_f} of Algorithm~\ref{scary:alg} and optimality condition \eqref{opt:z} we get
	\begin{align*}
	\sqn{v_f^{k+1} - v^*}
	&\leq
	\sqn{v_g^k - v^*}
	+
	2\sigma_2\<y^{k+1} - y^k,v_g^k - v^*>
	+
	3\sigma_2^2\sqn{y^{k+1} - y^k}
	\\&-
	2\zeta\< \mW(k) v_g^k,v_g^k - v^*>
    -
    \newu{2 \zeta_u\<\mAT (\nu^{-1}\mA v_g^k + \bb),v_g^k - v^*>}
	\\&+
	3\zeta^2\sqn{\mW(k)v_g^k}
    +
    \newu{3 \zeta_u^2 \sqn{\mAT(\nu^{-1}\mA v_g^k + \bb)}}
	\\&=
	\sqn{v_g^k - v^*}
	+
	2\sigma_2\<y^{k+1} - y^k,v_g^k - v^*>
	+
	3\sigma_2^2\sqn{y^{k+1} - y^k}
	\\&-
	2\zeta\< \mW(k)v_g^k,\mP v_g^k >
    -
    \newu{2 \zeta_u\<\mAT (\nu^{-1}\mA v_g^k + \bb),\mP_A (v_g^k - v^*)>}
	\\&+
	3\zeta^2\sqn{\mW(k)v_g^k}
    +
    \newu{3 \zeta_u^2 \sqn{\mAT(\nu^{-1}\mA v_g^k + \bb)}}.
	\end{align*}
	Using $\zeta$ definition \eqref{scary:zeta} we get
	\begin{align*}
	\sqn{v_f^{k+1} - v^*}
	&\leq
	\sqn{v_g^k - v^*}
	+
	2\sigma_2\<y^{k+1} - y^k,v_g^k - v^*>
	+
	3\sigma_2^2\sqn{y^{k+1} - y^k}
	\\&-
	2\zeta\< \mW(k)v_g^k,\mP v_g^k >
    -
    \newu{2 \zeta_u\<\mAT (\nu^{-1}\mA v_g^k + \bb),\mP_A(v_g^k - v^*)>}
	\\&+
	3\zeta^2\sqn{\mW(k)v_g^k}
    +
    \newu{3 \zeta_u^2 \sqn{\mAT(\nu^{-1}\mA v_g^k + \bb)}}.
    \\&=   
	\sqn{v_g^k - v^*}
	+
	2\sigma_2\<y^{k+1} - y^k,v_g^k - v^*>
	+
	3\sigma_2^2\sqn{y^{k+1} - y^k}
	\\&+
    \zeta \sqn{\mW(k) v_g^k - \mP v_g^k} 
    -
    \zeta \sqn{\mW(k) v_g^k}
    -
    \zeta \sqn{\mP v_g^k}
    \\&+
    % \newu{2 \zeta_u\<\mAT (\nu^{-1}\mA v_g^k + \bb),\mP_A(v_g^k - v^*)>}
    \newu{\zeta_u \sqn{\mAT (\nu^{-1}\mA v_g^k + \bb) - \mP_A(v_g^k - v^*)}
    - 
    \zeta_u \sqn{\mAT (\nu^{-1}\mA v_g^k + \bb)}}
    \\&-
    \newu{
    \zeta_u \sqn{\mP_A(v_g^k - v^*)}
    }
% 
	+
	3\zeta^2\sqn{\mW(k)v_g^k}
    +
    \newu{3 \zeta_u^2 \sqn{\mAT(\nu^{-1}\mA v_g^k + \bb)}}.
    \\&=   
	\sqn{v_g^k - v^*}
	+
	2\sigma_2\<y^{k+1} - y^k,v_g^k - v^*>
	+
	3\sigma_2^2\sqn{y^{k+1} - y^k}
	\\&+
    \frac13 \sqn{\mW(k) v_g^k - \mP v_g^k} 
    -
    \frac13 \sqn{\mP v_g^k}
    \\&+
    \newu{\frac13 \sqn{\mAT (\nu^{-1}\mA v_g^k + \bb) - \mP_A(v_g^k - v^*)}
    -
    \frac13 \sqn{\mP_A(v_g^k - v^*)}
    }
	\end{align*}
    Using condition \eqref{opt:u} we get 
	\begin{align*}
	\sqn{v_f^{k+1} - v^*}
	&\leq
	\sqn{v_g^k - v^*}
	+
	2\sigma_2\<y^{k+1} - y^k,v_g^k - v^*>
	+
	3\sigma_2^2\sqn{y^{k+1} - y^k}
	\\&+
    \frac13 \sqn{\mW(k) v_g^k - \mP v_g^k}
    -
    \frac13 \sqn{\mP v_g^k}
    \\&+
    \newu{\frac13 \sqn{\nu^{-1}\mAT \mA (v_g^k - v^*) - \mP_A(v_g^k - v^*)}
    -
    \frac13 \sqn{\mP_A(v_g^k - v^*)}
    }
	\end{align*}
	Using condition \eqref{eq:chi} and definition of $\chitA$ we get
	\begin{align*}
	\sqn{v_f^{k+1} - v^*}
	&\leq
	\sqn{v_g^k - v^*}
	+
	2\sigma_2\<y^{k+1} - y^k,v_g^k - v^*>
	+
	3\sigma_2^2\sqn{y^{k+1} - y^k}
	\\&-
    \frac1{3\chi} \sqn{v_g^k}_\mP
    -
    \newu{\frac1{3\chitA} \sqn{(v_g^k - v^*)}_{\mP_A} }
	\end{align*}
	Rearranging gives
	\begin{align*}
	-
	2\<y^{k+1} - y^k,v_g^k - v^*>
	&\leq
	\frac1{\sigma_2}\sqn{v_g^k - v^*}
    -
    \newu{\frac1{3\sigma_2\chitA} \sqn{(v_g^k - v^*)}_{\mP_A} }
    - 
	\frac1{\sigma_2}\sqn{v_f^{k+1} - v^*}
	\\&+
	3\sigma_2\sqn{y^{k+1} - y^k}
	-
    \frac1{3\sigma_2\chi} \sqn{v_g^k}_\mP
	\end{align*}
\end{proof} 

\begin{lemma}
    (New Lemma)
    \begin{equation}\label{scary:eq:u}
    \begin{split}
    \frac1{\gamma_u} \sqn{u^{k+1} - u^*} 
    &\leq 
    (\gamma_u^{-1} - \delta_u)\sqn{u^k - u^*} 
    + 
    \delta_u \sqn{u_g^k - u^*} 
    \\&+ 
    \delta_u(2 \gamma_u \delta_u - 1) \sqn{u_g^k - u^k}
    +
    2 \gamma_u \sqn{\nu^{-1}\mA v_g^k + \bb}
    \\&- 
    2 \nu^{-1} \<v_g^k - v^*, \mAT (u^k - u^*)>
    \end{split}
    \end{equation}
\end{lemma}
\begin{proof}
\begin{align*}
    \sqn{u^{k+1} - u^*} 
    &=
    \sqn{u^k - u^*}
    + 
    2 \<u^{k+1} - u^k, u^k - u^*>
    +
    \sqn{u^{k+1} - u^k}.
\end{align*}
Using Line \ref{scary:line:u} of Algorithm \ref{scary:alg} we get
\begin{align*}
    \sqn{u^{k+1} - u^*} 
    &\leq
    \sqn{u^k - u^*}
    + 
    2 \gamma_u \delta_u \<u_g^k - u^k, u^k - u^*>
    -
    2 \gamma_u  \<\nu^{-1} \mA v_g^k + \bb, u^k - u^*>
    \\&+
    2\gamma_u^2 \delta_u^2 \sqn{u_g^k - u^k}
    +
    2 \gamma_u^2 \sqn{\nu^{-1}\mA v_g^k + \bb}
    \\&=
    \sqn{u^k - u^*}
    + 
    \gamma_u \delta_u \sqn{u_g^k - u^*}
    -
    \gamma_u \delta_u \sqn{u_g^k - u^k}
    -
    \gamma_u \delta_u \sqn{u^k - u^*}
    \\&-
    2 \gamma_u  \<\nu^{-1} \mA v_g^k + \bb, u^k - u^*>
    +
    2\gamma_u^2 \delta_u^2 \sqn{u_g^k - u^k}
    +
    2 \gamma_u^2 \sqn{\nu^{-1}\mA v_g^k + \bb}.
    \\&=
    (1 - \gamma_u \delta_u) \sqn{u^k - u^*}
    + 
    \gamma_u \delta_u \sqn{u_g^k - u^*}
    +
    \gamma_u \delta_u(2\gamma_u \delta_u - 1) \sqn{u_g^k - u^k}
    \\&-
    2 \gamma_u  \<\nu^{-1} \mA v_g^k + \bb, u^k - u^*>
    +
    2 \gamma_u^2 \sqn{\nu^{-1}\mA v_g^k + \bb}.
\end{align*}
Using optimality condition \eqref{opt:u} and dividing both parts by $\gamma_u$ we get
\begin{align*}
    \frac1{\gamma_u} \sqn{u^{k+1} - u^*} 
    &\leq 
    (\gamma_u^{-1} - \delta_u)\sqn{u^k - u^*} 
    + 
    \delta_u \sqn{u_g^k - u^*} 
    \\&+ 
    \delta_u(2 \gamma_u \delta_u - 1) \sqn{u_g^k - u^k}
    +
    2 \gamma_u \sqn{\nu^{-1}\mA v_g^k + \bb}
    \\&- 
    2 \nu^{-1} \<v_g^k - v^*, \mAT (u^k - u^*)>.
\end{align*}


    
\end{proof}


\begin{lemma}
    (Lemma 10)
	Let $\delta, \delta_u$ be defined as follows:
	\begin{equation}\label{scary:delta}
	\delta = \frac{3}{25L}, \quad \delta_u = \frac{2 \delta \nu}{\chitA}.
	\end{equation}
	Let $\gamma, \gamma_u$ be defined as follows:
	\begin{equation}\label{scary:gamma}
	\gamma = \frac{\nu}{14\sigma_2\chi^2}, \quad
	\gamma_u = \frac{1}{4\sigma_2\chitA \chi}.
	\end{equation}
	Let $\theta$ be defined as follows:
	\begin{equation}\label{scary:theta}
	\theta = \frac{\nu}{4\sigma_2}.
	\end{equation}
	Let $\sigma_2$ be defined as follows:
	\begin{equation}\label{scary:sigma2}
	\sigma_2 = \frac{\sqrt{\mu}}{16\chi\sqrt{L}}.
	\end{equation}
	Let $\Psi_{yzu}^k$ be the following Lyapunov function
	\begin{equation}
	\begin{split}\label{scary:Psi_yzu}
	\Psi_{yzu}^k &= \left(\frac{1}{\theta} + \frac{\beta}{2}\right)\sqn{y^{k} - y^*}
	+
	\frac{\beta}{2\sigma_2}\sqn{y_f^{k} - y^*}
	+
	\frac{1}{\gamma}\sqn{\z^{k} - z^*}
	\\&+
    \newu{\frac1{\gamma_u}\sqn{u^k - u^*}}
    +
	\frac{4}{3\gamma}\sqn{m^{k}}_\mP
	+
	\frac{\nu^{-1}}{\sigma_2}\sqn{v_f^{k} - v^*}.
	\end{split}
	\end{equation}
	Then the following inequality holds:
	\begin{equation}\label{scary:eq:yz}
	\Psi_{yzu}^{k+1} \leq \left(1 - \frac{\sqrt{\mu}}{32\chi\sqrt{L}}\right)\Psi_{yz}^k
	+
	\bg_F(x_g^k, x^*) - \frac{\nu}{2}\sqn{x_g^k - x^*}
	-
	2\<x^{k+1} - x^*, y^{k+1} - y^*>.
	\end{equation}
\end{lemma}
\begin{proof}
	Combining \eqref{scary:eq:y}, \eqref{scary:eq:z} and \eqref{scary:eq:u} gives
 
	\begin{align*}
	\MoveEqLeft[4]\left(\frac{1}{\theta} + \frac{\beta}{2}\right)\sqn{y^{k+1} - y^*}
	+
	\frac{\beta}{2\sigma_2}\sqn{y_f^{k+1} - y^*}
	+
	\frac{1}{\gamma}\sqn{\z^{k+1} - z^*}
    +
    \newu{\frac1{\gamma_u} \sqn{u^{k+1} - u^*}}
	+
	\frac{4}{3\gamma}\sqn{m^{k+1}}_\mP
	\\&\leq
	\left(\frac{1}{\gamma} - \delta\right)\sqn{\z^k - z^*}
	+
	\left(1-(4\chi)^{-1}+\frac{3\gamma\delta}{2}\right)\frac{4}{3\gamma}\sqn{m^k}_\mP
	+
	\frac{1}{\theta}\sqn{y^k - y^*}
	+
	\frac{\beta(1-\sigma_2/2)}{2\sigma_2}\sqn{y_f^k - y^*}
	\\&-
	2\nu^{-1}\<v_g^k - v^*, y^k + z^k - (y^* + z^*)>
	-
	2\nu^{-1}\<v_g^k - v^*, y^{k+1} - y^k>
	\\&+
	\gamma\nu^{-2}\left(1 + 6\chi\right)\sqn{v_g^k}_\mP
	+
	\left(\frac{\beta\sigma_2^2}{4} - \frac{1}{\theta}\right)\sqn{y^{k+1} - y^k}
	+
	2\delta\sqn{z_g^k  - z^*}
	-
	\frac{\beta}{4}\sqn{y_g^k - y^*}
	\\&+
	\bg_F(x_g^k, x^*) - \frac{\nu}{2}\sqn{x_g^k - x^*}
	-
	2\<x^{k+1} - x^*, y^{k+1} - y^*>
	+\left(2\gamma\delta^2-\delta\right)\sqn{z_g^k - z^k}
    \\&+ \newu{
    (\gamma_u^{-1} - \delta_u)\sqn{u^k - u^*} 
    + 
    \delta_u \sqn{u_g^k - u^*} 
    + 
    \delta_u(2 \gamma_u \delta_u - 1) \sqn{u_g^k - u^k}
    +
    2 \gamma_u \sqn{\nu^{-1}\mA v_g^k + \bb}
    }
    \\&- 
    \newu{2 \nu^{-1} \<v_g^k - v^*, \mAT (u^k - u^*)>}
    \\&=
	\left(\frac{1}{\gamma} - \delta\right)\sqn{\z^k - z^*}
	+
	\left(1-(4\chi)^{-1}+\frac{3\gamma\delta}{2}\right)\frac{4}{3\gamma}\sqn{m^k}_\mP
	+
	\frac{1}{\theta}\sqn{y^k - y^*}
	+
	\frac{\beta(1-\sigma_2/2)}{2\sigma_2}\sqn{y_f^k - y^*}
	\\&-
	\changed{2\nu^{-1}\<v_g^k - v^*, v^k - v^*>}
	-
	2\nu^{-1}\<v_g^k - v^*, y^{k+1} - y^k>
	\\&+
	\gamma\nu^{-2}\left(1 + 6\chi\right)\sqn{v_g^k}_\mP
	+
	\left(\frac{\beta\sigma_2^2}{4} - \frac{1}{\theta}\right)\sqn{y^{k+1} - y^k}
	+
	2\delta\sqn{z_g^k  - z^*}
	-
	\frac{\beta}{4}\sqn{y_g^k - y^*}
	\\&+
	\bg_F(x_g^k, x^*) - \frac{\nu}{2}\sqn{x_g^k - x^*}
	-
	2\<x^{k+1} - x^*, y^{k+1} - y^*>
	+\left(2\gamma\delta^2-\delta\right)\sqn{z_g^k - z^k}
    \\&+ \newu{
    (\gamma_u^{-1} - \delta_u)\sqn{u^k - u^*} 
    + 
    \delta_u \sqn{u_g^k - u^*} 
    + 
    \delta_u(2 \gamma_u \delta_u - 1) \sqn{u_g^k - u^k}
    +
    2 \gamma_u \sqn{\nu^{-1}\mA v_g^k + \bb}
    }.
	\end{align*}
	Using \eqref{scary:eq:3} and \eqref{scary:eq:4} we get
	\begin{align*}
	\MoveEqLeft[4]\left(\frac{1}{\theta} + \frac{\beta}{2}\right)\sqn{y^{k+1} - y^*}
	+
	\frac{\beta}{2\sigma_2}\sqn{y_f^{k+1} - y^*}
	+
	\frac{1}{\gamma}\sqn{\z^{k+1} - z^*}
    +
    \newu{\frac1{\gamma_u} \sqn{u^{k+1} - u^*}}
	+
	\frac{4}{3\gamma}\sqn{m^{k+1}}_\mP
	\\&\leq
	\left(\frac{1}{\gamma} - \delta\right)\sqn{\z^k - z^*}
	+
	\left(1-(4\chi)^{-1}+\frac{3\gamma\delta}{2}\right)\frac{4}{3\gamma}\sqn{m^k}_\mP
	+
	\frac{1}{\theta}\sqn{y^k - y^*}
	+
	\frac{\beta(1-\sigma_2/2)}{2\sigma_2}\sqn{y_f^k - y^*}
	\\&-
%
	\changed{
	2\nu^{-1}\sqn{v_g^k - v^*}
	+
	\frac{\nu^{-1}(1-\sigma_2/2)}{\sigma_2}\left(\sqn{v_f^k - v^*} - \sqn{v_g^k - v^*} \right)
    }
%
    \\&+ \changed{
	\frac{\nu^{-1}}{\sigma_2}\sqn{v_g^k - v^*}
	-
	\newu{\frac{\nu^{-1}}{2\sigma_2 \chitA}\sqn{v_g^k - v^*}_{\mP_A}}
	-
	\frac{\nu^{-1}}{\sigma_2}\sqn{v_f^{k+1} - v^*}
    }
	+ \changed{
	2\nu^{-1}\sigma_2\sqn{y^{k+1} - y^k}
	-
	\frac{\nu^{-1}}{2\sigma_2\chi}\sqn{v_g^k}_{\mP}
    }
%
	\\&+
	\gamma\nu^{-2}\left(1 + 6\chi\right)\sqn{v_g^k}_\mP
	+
	\left(\frac{\beta\sigma_2^2}{4} - \frac{1}{\theta}\right)\sqn{y^{k+1} - y^k}
	+
	2\delta\sqn{z_g^k  - z^*}
	-
	\frac{\beta}{4}\sqn{y_g^k - y^*}
	\\&+
	\bg_F(x_g^k, x^*) - \frac{\nu}{2}\sqn{x_g^k - x^*}
	-
	2\<x^{k+1} - x^*, y^{k+1} - y^*>
	+\left(2\gamma\delta^2-\delta\right)\sqn{z_g^k - z^k}
    \\&+ \newu{
    (\gamma_u^{-1} - \delta_u)\sqn{u^k - u^*} 
    + 
    \delta_u \sqn{u_g^k - u^*} 
    + 
    \delta_u(2 \gamma_u \delta_u - 1) \sqn{u_g^k - u^k}
    +
    2 \gamma_u \sqn{\nu^{-1}\mA v_g^k + \bb}
    }
%
	\\&=
	\left(\frac{1}{\gamma} - \delta\right)\sqn{\z^k - z^*}
	+
	\left(1-(4\chi)^{-1}+\frac{3\gamma\delta}{2}\right)\frac{4}{3\gamma}\sqn{m^k}_\mP
	+
	\frac{1}{\theta}\sqn{y^k - y^*}
	+
	\frac{\beta(1-\sigma_2/2)}{2\sigma_2}\sqn{y_f^k - y^*}
	\\&+
%
	\frac{\nu^{-1}(1-\sigma_2/2)}{\sigma_2}\sqn{v_f^k - v^*}
	-
	\frac{\nu^{-1}}{\sigma_2}\sqn{v_f^{k+1} - v^*}
	+
	2\delta\sqn{z_g^k  - z^*}
    + 
    \newu{\delta_u \sqn{u_g^k - u^*}}
%
    \\&-
	\frac{\beta}{4}\sqn{y_g^k - y^*}
	-
    \changed{\frac{3\nu^{-1}}{2}}\sqn{v_g^k - v^*}
%
    +
	\changed{\left(\gamma\nu^{-2}\left(1 + 6\chi\right)-
	\frac{\nu^{-1}}{2\sigma_2\chi} \right)}\sqn{v_g^k}_\mP
%
    \\& -
	\newu{\frac{\nu^{-1}}{2\sigma_2 \chitA}\sqn{v_g^k - v^*}_{\mP_A}}
	+
	\changed{\left(\frac{\beta\sigma_2^2}{4} + 2\nu^{-1}\sigma_2 - \frac{1}{\theta}\right)}\sqn{y^{k+1} - y^k}
	\\&+
	\bg_F(x_g^k, x^*) - \frac{\nu}{2}\sqn{x_g^k - x^*}
	-
	2\<x^{k+1} - x^*, y^{k+1} - y^*>
	+\left(2\gamma\delta^2-\delta\right)\sqn{z_g^k - z^k}
    \\&+ \newu{
    (\gamma_u^{-1} - \delta_u)\sqn{u^k - u^*} 
    + 
    \delta_u(2 \gamma_u \delta_u - 1) \sqn{u_g^k - u^k}
    +
    2 \gamma_u \sqn{\nu^{-1}\mA v_g^k + \bb}
    }
	\end{align*}
	Using $\beta$ definition \eqref{scary:beta} and $\nu$ definition \eqref{scary:nu} we get
	\begin{align*}
	\MoveEqLeft[4]\left(\frac{1}{\theta} + \frac{\beta}{2}\right)\sqn{y^{k+1} - y^*}
	+
	\frac{\beta}{2\sigma_2}\sqn{y_f^{k+1} - y^*}
	+
	\frac{1}{\gamma}\sqn{\z^{k+1} - z^*}
    +
    \newu{\frac1{\gamma_u} \sqn{u^{k+1} - u^*}}
	+
	\frac{4}{3\gamma}\sqn{m^{k+1}}_\mP
	\\&\leq
	\left(\frac{1}{\gamma} - \delta\right)\sqn{\z^k - z^*}
	+
	\left(1-(4\chi)^{-1}+\frac{3\gamma\delta}{2}\right)\frac{4}{3\gamma}\sqn{m^k}_\mP
	+
	\frac{1}{\theta}\sqn{y^k - y^*}
	+
	\frac{\beta(1-\sigma_2/2)}{2\sigma_2}\sqn{y_f^k - y^*}
	\\&+
	\frac{\nu^{-1}(1-\sigma_2/2)}{\sigma_2}\sqn{v_f^k - v^*} 
	-
	\frac{\nu^{-1}}{\sigma_2}\sqn{v_f^{k+1} - v^*}
	+
	2\delta\sqn{z_g^k  - z^*}
    + 
    \newu{\delta_u \sqn{u_g^k - u^*}}
    \\&-
	\changed{\frac{1}{8L}}\sqn{y_g^k - y^*}
	-
    \changed{\frac{3}{\mu}}\sqn{v_g^k - v^*}
    +
	\left(\gamma\nu^{-2}\left(1 + 6\chi\right)-
	\frac{\nu^{-1}}{2\sigma_2\chi} \right)\sqn{v_g^k}_\mP
    \\& -
	\newu{\frac{\nu^{-1}}{2\sigma_2 \chitA}\sqn{v_g^k - v^*}_{\mP_A}}
	+
	\left(\frac{\beta\sigma_2^2}{4} + 2\nu^{-1}\sigma_2 - \frac{1}{\theta}\right)\sqn{y^{k+1} - y^k}
	\\&+
	\bg_F(x_g^k, x^*) - \frac{\nu}{2}\sqn{x_g^k - x^*}
	-
	2\<x^{k+1} - x^*, y^{k+1} - y^*>
	+\left(2\gamma\delta^2-\delta\right)\sqn{z_g^k - z^k}
    \\&+ \newu{
    (\gamma_u^{-1} - \delta_u)\sqn{u^k - u^*} 
    + 
    \delta_u(2 \gamma_u \delta_u - 1) \sqn{u_g^k - u^k}
    +
    2 \gamma_u \sqn{\nu^{-1}\mA v_g^k + \bb}
    }
    \end{align*}
    Using $\delta$ and $\delta_u$ definitions \eqref{scary:delta}  we get
    TODO: explain
	\begin{align*}
	\MoveEqLeft[4]\left(\frac{1}{\theta} + \frac{\beta}{2}\right)\sqn{y^{k+1} - y^*}
	+
	\frac{\beta}{2\sigma_2}\sqn{y_f^{k+1} - y^*}
	+
	\frac{1}{\gamma}\sqn{\z^{k+1} - z^*}
    +
    \newu{\frac1{\gamma_u} \sqn{u^{k+1} - u^*}}
	+
	\frac{4}{3\gamma}\sqn{m^{k+1}}_\mP
	\\&\leq
	\left(\frac{1}{\gamma} - \delta\right)\sqn{\z^k - z^*}
	+
	\left(1-(4\chi)^{-1}+\frac{3\gamma\delta}{2}\right)\frac{4}{3\gamma}\sqn{m^k}_\mP
	+
	\frac{1}{\theta}\sqn{y^k - y^*}
	+
	\frac{\beta(1-\sigma_2/2)}{2\sigma_2}\sqn{y_f^k - y^*}
	\\&+
	\frac{\nu^{-1}(1-\sigma_2/2)}{\sigma_2}\sqn{v_f^k - v^*}  
	-
	\frac{\nu^{-1}}{\sigma_2}\sqn{v_f^{k+1} - v^*}
    +
	\left(\gamma\nu^{-2}\left(1 + 6\chi\right)-
	\frac{\nu^{-1}}{2\sigma_2\chi} \right)\sqn{v_g^k}_\mP
    \\& -
	\newu{\frac{\nu^{-1}}{2\sigma_2 \chitA}\sqn{v_g^k - v^*}_{\mP_A}}
	+
	\left(\frac{\beta\sigma_2^2}{4} + 2\nu^{-1}\sigma_2 - \frac{1}{\theta}\right)\sqn{y^{k+1} - y^k}
	\\&+
	\bg_F(x_g^k, x^*) - \frac{\nu}{2}\sqn{x_g^k - x^*}
	-
	2\<x^{k+1} - x^*, y^{k+1} - y^*>
	+\left(2\gamma\delta^2-\delta\right)\sqn{z_g^k - z^k}
    \\&+ \newu{
    (\gamma_u^{-1} - \delta_u)\sqn{u^k - u^*} 
    + 
    \delta_u(2 \gamma_u \delta_u - 1) \sqn{u_g^k - u^k}
    +
    2 \gamma_u \sqn{\nu^{-1}\mA v_g^k + \bb}
    }
    \end{align*}
	Using $\gamma$ definition \eqref{scary:gamma} we get
	\begin{align*}
	\MoveEqLeft[4]\left(\frac{1}{\theta} + \frac{\beta}{2}\right)\sqn{y^{k+1} - y^*}
	+
	\frac{\beta}{2\sigma_2}\sqn{y_f^{k+1} - y^*}
	+
	\frac{1}{\gamma}\sqn{\z^{k+1} - z^*}
    +
    \newu{\frac1{\gamma_u} \sqn{u^{k+1} - u^*}}
	+
	\frac{4}{3\gamma}\sqn{m^{k+1}}_\mP
	\\&\leq
	\left(\frac{1}{\gamma} - \delta\right)\sqn{\z^k - z^*}
	+
	\left(1-(4\chi)^{-1}+\frac{3\gamma\delta}{2}\right)\frac{4}{3\gamma}\sqn{m^k}_\mP
	+
	\frac{1}{\theta}\sqn{y^k - y^*}
	+
	\frac{\beta(1-\sigma_2/2)}{2\sigma_2}\sqn{y_f^k - y^*}
	\\&+
	\frac{\nu^{-1}(1-\sigma_2/2)}{\sigma_2}\sqn{v_f^k - v^*} 
	-
	\frac{\nu^{-1}}{\sigma_2}\sqn{v_f^{k+1} - v^*}
    \\& -
	\newu{\frac{\nu^{-1}}{2\sigma_2 \chitA}\sqn{v_g^k - v^*}_{\mP_A}}
	+
	\left(\frac{\beta\sigma_2^2}{4} + 2\nu^{-1}\sigma_2 - \frac{1}{\theta}\right)\sqn{y^{k+1} - y^k}
	\\&+
	\bg_F(x_g^k, x^*) - \frac{\nu}{2}\sqn{x_g^k - x^*}
	-
	2\<x^{k+1} - x^*, y^{k+1} - y^*>
	+\left(2\gamma\delta^2-\delta\right)\sqn{z_g^k - z^k}
    \\&+ \newu{
    (\gamma_u^{-1} - \delta_u)\sqn{u^k - u^*} 
    + 
    \delta_u(2 \gamma_u \delta_u - 1) \sqn{u_g^k - u^k}
    +
    2 \gamma_u \sqn{\nu^{-1}\mA v_g^k + \bb}
    }
    \end{align*}
    Using (TODO: remove $A_nu$ from everywhere)
    \begin{equation*}
        \sqn{\mA_nu(v_g^k - v^*)} \leq \sigma^2_{max}(\mA) \sqn{v_g^k - v^*}_{\mP_A} = \nu \sqn{v_g^k - v^*}_{\mP_A}
    \end{equation*}
    and $\gamma_u$ definition we get
	\begin{align*}
	\MoveEqLeft[4]\left(\frac{1}{\theta} + \frac{\beta}{2}\right)\sqn{y^{k+1} - y^*}
	+
	\frac{\beta}{2\sigma_2}\sqn{y_f^{k+1} - y^*}
	+
	\frac{1}{\gamma}\sqn{\z^{k+1} - z^*}
    +
    \newu{\frac1{\gamma_u} \sqn{u^{k+1} - u^*}}
	+
	\frac{4}{3\gamma}\sqn{m^{k+1}}_\mP
	\\&\leq
	\left(\frac{1}{\gamma} - \delta\right)\sqn{\z^k - z^*}
	+
	\left(1-(4\chi)^{-1}+\frac{3\gamma\delta}{2}\right)\frac{4}{3\gamma}\sqn{m^k}_\mP
	+
	\frac{1}{\theta}\sqn{y^k - y^*}
	+
	\frac{\beta(1-\sigma_2/2)}{2\sigma_2}\sqn{y_f^k - y^*}
	\\&+
	\frac{\nu^{-1}(1-\sigma_2/2)}{\sigma_2}\sqn{v_f^k - v^*}  
	-
	\frac{\nu^{-1}}{\sigma_2}\sqn{v_f^{k+1} - v^*}
    \\& +
	\left(\frac{\beta\sigma_2^2}{4} + 2\nu^{-1}\sigma_2 - \frac{1}{\theta}\right)\sqn{y^{k+1} - y^k}
	\\&+
	\bg_F(x_g^k, x^*) - \frac{\nu}{2}\sqn{x_g^k - x^*}
	-
	2\<x^{k+1} - x^*, y^{k+1} - y^*>
	+\left(2\gamma\delta^2-\delta\right)\sqn{z_g^k - z^k}
    \\&+ \newu{
    (\gamma_u^{-1} - \delta_u)\sqn{u^k - u^*} 
    + 
    \delta_u(2 \gamma_u \delta_u - 1) \sqn{u_g^k - u^k}
    }
    \end{align*}
 	Using $\theta$ definition together with \eqref{scary:nu}, \eqref{scary:beta} and \eqref{scary:sigma2} gives
	\begin{align*}
	\MoveEqLeft[4]\left(\frac{1}{\theta} + \frac{\beta}{2}\right)\sqn{y^{k+1} - y^*}
	+
	\frac{\beta}{2\sigma_2}\sqn{y_f^{k+1} - y^*}
	+
	\frac{1}{\gamma}\sqn{\z^{k+1} - z^*}
    +
    \newu{\frac1{\gamma_u} \sqn{u^{k+1} - u^*}}
	+
	\frac{4}{3\gamma}\sqn{m^{k+1}}_\mP
	\\&\leq
	\left(\frac{1}{\gamma} - \delta\right)\sqn{\z^k - z^*}
	+
	\left(1-(4\chi)^{-1}+\frac{3\gamma\delta}{2}\right)\frac{4}{3\gamma}\sqn{m^k}_\mP
	+
	\frac{1}{\theta}\sqn{y^k - y^*}
	+
	\frac{\beta(1-\sigma_2/2)}{2\sigma_2}\sqn{y_f^k - y^*}
	\\&+
	\frac{\nu^{-1}(1-\sigma_2/2)}{\sigma_2}\sqn{v_f^k - v^*}
	-
	\frac{\nu^{-1}}{\sigma_2}\sqn{v_f^{k+1} - v^*}
	\\&+
	\bg_F(x_g^k, x^*) - \frac{\nu}{2}\sqn{x_g^k - x^*}
	-
	2\<x^{k+1} - x^*, y^{k+1} - y^*>
	+\left(2\gamma\delta^2-\delta\right)\sqn{z_g^k - z^k}
    \\&+ \newu{
    (\gamma_u^{-1} - \delta_u)\sqn{u^k - u^*} 
    + 
    \delta_u(2 \gamma_u \delta_u - 1) \sqn{u_g^k - u^k}
    }
    \end{align*}
    Using $\gamma$ definition \eqref{scary:gamma} with $\delta$ definition \eqref{scary:delta} and $\gamma_u$ definition with $\delta_u$ definition we get
	\begin{align*}
	\MoveEqLeft[4]\left(\frac{1}{\theta} + \frac{\beta}{2}\right)\sqn{y^{k+1} - y^*}
	+
	\frac{\beta}{2\sigma_2}\sqn{y_f^{k+1} - y^*}
	+
	\frac{1}{\gamma}\sqn{\z^{k+1} - z^*}
    +
    \newu{\frac1{\gamma_u} \sqn{u^{k+1} - u^*}}
	+
	\frac{4}{3\gamma}\sqn{m^{k+1}}_\mP
	\\&\leq
	\left(\frac{1}{\gamma} - \delta\right)\sqn{\z^k - z^*}
	+
	\left(1-(8\chi)^{-1}\right)\frac{4}{3\gamma}\sqn{m^k}_\mP
	+
	\frac{1}{\theta}\sqn{y^k - y^*}
	+
	\frac{\beta(1-\sigma_2/2)}{2\sigma_2}\sqn{y_f^k - y^*}
	\\&+
	\frac{\nu^{-1}(1-\sigma_2/2)}{\sigma_2}\sqn{v_f^k - v^*} 
	-
	\frac{\nu^{-1}}{\sigma_2}\sqn{v_f^{k+1} - v^*}
	\\&+
	\bg_F(x_g^k, x^*) - \frac{\nu}{2}\sqn{x_g^k - x^*}
	-
	2\<x^{k+1} - x^*, y^{k+1} - y^*>
    + 
    \newu{(\gamma_u^{-1} - \delta_u)\sqn{u^k - u^*}}
    \end{align*}
    After rearranging and using $\Psi_{yzu}^k$ definition \eqref{scary:Psi_yzu} we get
    \begin{align*}
	\Psi_{yzu}^{k+1} 
	&\leq
	\max\left\{(1 + \theta\beta/2)^{-1}, (1-\gamma\delta), \newu{(1-\gamma_u \delta_u)}, (1-\sigma_2/2), (1-(8\chi)^{-1})\right\}\Psi_{yz}^k
	\\&+
	\bg_F(x_g^k, x^*) - \frac{\nu}{2}\sqn{x_g^k - x^*}
	-
	\\&\leq
	\max\left\{1 - \frac{\sqrt{\mu}}{32\chi\sqrt{L}},~ \newu{1- \frac{12 \sqrt\mu}{25\chitA^2 \sqrt L}}\right\}\Psi_{yzu}^k
	+
	\bg_F(x_g^k, x^*) - \frac{\nu}{2}\sqn{x_g^k - x^*}
	-
	2\<x^{k+1} - x^*, y^{k+1} - y^*>.
	\end{align*}
\end{proof}


==> review_response.tex <==
Reviewer Comments:

Reviewer 1
This paper considers affine-constrained problems. The authors present a new linearly convergent dual algorithm for decentralized affine-constrained optimization of the sum of smooth strongly convex functions over time-varying networks. The paper has been well organized and presented and the subject of the paper appears to be interesting to the readers of the Computational Management Science. This paper has a solid theoretical contribution and also another strong point of the manuscript is the fact that, the findings are supported by numerical experiments. Overall, this paper can be of value for researchers interested in decentralized optimization problems and I believe it deserves a publication in Computational Management Science. I suggest that this paper is accepted with the following minor revisions.

Minor comments:

1) The authors should correct a few mistakes in the English syntax. For example:

 - in page 10, correct the expression "what is rather close".
 - in page 11, correct the expression "This means that cannot apply our approach".

2) The literature review in the introduction section could be described more thoroughly by, e.g., shortly describing applications of decentralized optimization in high-dimensional machine learning problems and also control drone swarms.

3) Although, the computational results are encouraging, perhaps the authors could elaborate more in this section and provide a few further technical details about, e.g., the instances, the computational infrastructure, etc

Reviewer 2
The authors in this paper study a distributed optimization paradigm when the agents additionally have local affine constraints and the communication graph can change over time. They developed the first linearly convergent decentralized algorithm for time-varying networks by generalizing the optimal decentralized algorithm ADOM to the case of affine constraints. Accordingly, they show that its rate of convergence is optimal for first-order methods by providing the lower bounds for the number of communications and oracle calls. Numerical experiments were also conducted to show the efficiency and efficacy of the algorithm. Well done.

-----

Response

Reviewer 1
1. We have corrected these, along with other observed errors in the text.
2. This part of the introduction has been slightly extended, and a handful of references to application-related papers were added
3. We have posted the source code of the experiments on GitHub and inserted the link in the text, so that the reader can get information about any technical details from there.
--
